Quasi-Monte Carlo Variational Inference

Many machine learning problems involve Monte Carlo gradient estimators. As a prominent example, we focus on Monte Carlo variational inference (MCVI) in this paper. The performance of MCVI crucially depends on the variance of its stochastic gradients. We propose variance reduction by means of Quasi-Monte Carlo (QMC) sampling. QMC replaces N i.i.d. samples from a uniform probability distribution by a deterministic sequence of samples of length N. This sequence covers the underlying random variable space more evenly than i.i.d. draws, reducing the variance of the gradient estimator. With our novel approach, both the score function and the reparameterization gradient estimators lead to much faster convergence. We also propose a new algorithm for Monte Carlo objectives, where we operate with a constant learning rate and increase the number of QMC samples per iteration. We prove that this way, our algorithm can converge asymptotically at a faster rate than SGD. We furthermore provide theoretical guarantees on QMC for Monte Carlo objectives that go beyond MCVI, and support our findings by several experiments on large-scale data sets from various domains.

==> backup_qmc_writeup.tex <==
\subsection{Quasi Monte Carlo} \label{sec:QMC}
Low discrepancy sequences (also called quasi Monte Carlo sequences), are used
to approximate integrals over the $[0,1]^d$ hyper-cube:
\begin{eqnarray*}
\EE{\psi(U)} = \int_{[0,1]^d} \psi(u) du, 
\end{eqnarray*}
that is the expectation of the random variable $ \psi(U)$, where $ U \sim
\mathcal{U} \left([0,1]^d \right)$. The basic Monte Carlo approximation of the
integral is  $\hat{I}_N := \frac{1}{N}
\sumnN \psi(\uvec_n)$, where each $\uvec_n\sim \mathcal{U} \left([0,1]^d \right)$. 
The error of this approximation is $\Op(N^{-1/2})$, since 
$\Var[\hat{I}_N] = \Var[\psi(U)]/N$. 

It is possible to improve on this basic approximation, by replacing the random variables $\uvec_n$ 
by a so called low-discrepancy sequence; that is, informally, a deterministic sequence that covers 
$[0,1]^d$ more regularly. See the appendix for a formal definition of the star discrepancy 
$D^*(\uvec_{1:N})$. 

The importance of the notion of discrepancy and in particular the star discrepancy
is highlighted by the Koksma-Hlawka inequality, which allows to relate the error
of the integration to the coverage of the space and the total variation of the
function that is integrated: 
\begin{eqnarray*}
\left| \int_{[0,1]^d} \psi(\uvec) d\uvec -  \frac{1}{N} \sumnN \psi(\uvec_n) \right| \leq V(\psi) D^*(\uvec_{1:N}), 
\end{eqnarray*}
where $V(\psi)$ is the total variation in the sense of Hardy and Krause. 
This quantity is closely linked to the smoothness of the function $\psi$; 
see \cite{kuipers2012uniform} and \cite{leobacher2014introduction} for more details. 

It is possible to construct sequences $\uvec_n$ such that when $N$ is fixed in
advance $D^*(\uvec_{1:N})$ is $\mathcal{O}\left( N^{-1}(\log N)^{d-1} \right)$
and when $N$ is allowed to grow, i.e., the sequence can be generated
iteratively, then $D^*(\uvec_{1:N}) = \mathcal{O}\left( N^{-1}(\log N)^{d}
\right)$. Then $\forall \tau > 0$ the error rate is
$\mathcal{O}\left(N^{-1+\tau} \right)$ for the QMC integration. 
Consequently, QMC integration schemes are asymptotically more efficient than MC
schemes. 
We observe in practice that QMC integration outperforms MC integration even 
for small $N$ in most applications, see e.g. the examples in Chapter X of \cite{glasserman2013monte}.

A drawback of QMC is that it does not come with an easy way 
to assess the uncertainty of an approximation. 

This motivates the idea of randomized quasi Monte Carlo (RQMC). 
The reintroduction of randomness in a low discrepancy sequence while preserving
the low discrepancy of that sequence enables the construction of confidence
intervals. The simplest method for this purpose is to use a randomly shifted
sequence. Let $v \sim \mathcal{U}([0,1]^d)$. Then the sequence based on
\begin{eqnarray*}
\hat{\uvec}_n :=  \uvec_n + v \mod 1
\end{eqnarray*}
preserves the properties of the low discrepancy sequence with probability $1$
and is marginally uniformly distributed. Consequently, confidence intervals
based on repeated sampling may be obtained. Moreover, the introduction of randomness makes
the approximation unbiased, which is not the case for an entirely deterministic approximation.

A more sophisticated approach has been introduced by
\cite{owen_scrambled_1997}, who proposed to inject randomness in the
construction of the low discrepancy sequences and obtains so called
scrambled nets, that are also marginally uniformly distributed. The main advantage of this approach is that under the
assumption of smoothness of the derivatives of the function, the speed of
convergence can be even further improved as stated in the appendix. 
In words, $\forall \tau > 0$ the RQMC error rate is $\OO(N^{-3/2+\tau})$ when
a scrambled net is used.
%$(\lambda, t, m, d)-$

\subsection{RQMC for stochastic optimization}
In what follows we show that using RQMC within variational inference is beneficial to the optimization routine. 
However, our results are more general, therefore we state our results in a more general sense. 
The aim of stochastic optimization is to find the optima of a function $\F: \lambdavec  \in \Theta \rightarrow \RR$, where the optimizer has only access to a noisy version of the function, e.g. $ \Fest (\lambdavec)$, where $\EE_Z [\Fest (\lambdavec)] = \F(\lambdavec) ~ \forall \lambdavec$ and where $Z \sim q_{\lambdavec}(z)$ is the stochastic perturbation of the function. The optimum of the function is defined as $\lambdavec^\star \in \arg\min_{\lambdavec} \EE_Z [\Fest (\lambdavec)]$. 
We also have access to noisy gradients of the function, denoted by $\nabla \Fest(\lambdavec)$, where we assume that $\EE_Z[\nabla \Fest(\lambdavec)] = \nabla \F(\lambdavec)$. More specifically we suppose that for every $\lambdavec$, we are able to generate a sequence of random variables $z_1, \cdots, z_N \sim q_{\lambdavec}(z)$ such that unbiased estimators for $\F(\lambdavec)$ and $\nabla \F(\lambdavec)$ are given as 
$$
\FestN(\lambdavec) = \frac{1}{N} \sumnN \F_{z_n}(\lambdavec), ~  \nabla \FestN(\lambdavec) = \frac{1}{N} \sumnN \nabla \F_{z_n}(\lambdavec).
$$
In the context of variational inference the defined quantities are equivalent to 
$\FestN(\lambdavec) = - \ELBOestN(\lambdavec)$, $\nabla \FestN(\lambdavec) = - \nabla \ELBOestN(\lambdavec)$ and
$\nabla \F_{z_n}(\lambdavec) = -f(z_n| \lambdavec)$
or its reparametrized version, respectively. The negative sign is due to the convention of studying the minimization of general objective functions. 
A common way to find the optimal value $\lambdavec^\star$ is to use stochastic approximations as for example stochastic gradient descent as defined via the update rule
\begin{equation} \label{eq:sgd_update}
\lambdavec_{t+1} = \lambdavec_{t} - \alpha \nabla \FestN(\lambdavec_{t}),
\end{equation}
for a small learning rate $\alpha$ that is iterated until $|\FestN(\lambdavec_{t})-\FestN(\lambdavec_{t+1})|\leq \epsilon$, for a small threshold $\epsilon$. However, the quality of the approximation $\lambdavec_{T} \approx \lambdavec^\star$ crucially depends on the variance of the estimator $\nabla \FestN$, see \cite{johnson2013accelerating} for instance. 

In what follows, we study the setting where the simulation of $z_n \sim q_{\lambdavec}(z)$ is achieved via the transformation of a RQMC sequence. Therefore we introduce the transformation 
$\Gamma(\uvec_n) = z_n$, where $\Gamma$ is for example the quantile function. 
We will show that when a RQMC sequence is used for generating $z_1, \cdots, z_N$, the so obtained reduction in variance is beneficial to the optimization procedure defined in \eqref{eq:sgd_update}. 
Intuitively, the variance of $\nabla \FestN(\lambdavec)$ based on a RQMC sequence will be of order $\oo(N^{-1})$ and thus for $N$ large enough, the variance will be smaller than for the MC counterpart, that is of order $N^{-1}$.
We study the case of a Lipschitz continuous functions and strongly convex functions with fixed step size. More challenging theoretical frameworks as for example decreasing step sizes or adaptive step sizes are left to future investigation. 

\subsection{Stochastic gradient descent with fixed step size}
In the case of function with Lipschitz continous derivates we obtain the following result. 
\begin{theorem} \label{theorem:lipschitz_functions}
Let $\F$ be a function with Lipschitz continuous derivatives, e.g. there exists $L>0$ s.t. $\forall \lambdavec, \overline{\lambdavec}$ $\norm{ \nabla \F(\lambdavec) - \nabla \F(\overline{\lambdavec}) } \leq L \norm{\lambdavec - \overline{\lambdavec} }$, let $U_N = \{\uvec_1, \cdots, \uvec_N\}$ be a RQMC sequence and let $ \forall \lambdavec$ $G: \uvec \rightarrow \nabla \F_{\Gamma(\uvec)}(\lambdavec)$ satisfy the conditions of Theorem \ref{theorem:owen}. Let $\alpha < 2/L$ and let $\mu = 1 - \alpha L/2$. 
Then  
$\tr \Var_{U_N}[ \nabla \FestN(\lambdavec)] \leq M_V \times r(N) \forall \lambdavec$, where $M_V < \infty$ and $r(N)=\oo\left(N^{-1}\right)$ and
\begin{eqnarray*} \label{eq:sum_lipschitz}
\frac{\sumtT \EE \norm{ \nabla \F(\lambdavec_t)}}{T} \leq \frac{1}{2 \mu} \alpha L  M_V r(N) + \\
 \frac{ \F(\lambdavec_1) - \EE[ \F(\lambdavec_T)] }{\alpha \mu T }.
\end{eqnarray*}
Consequently, 
\begin{equation} \label{eq:limit_lipschitz}
\limT \frac{\sumtT \EE \norm{ \nabla \F(\lambdavec_t)}}{T} \leq \frac{1}{2 \mu} \alpha L  M_V r(N) .
\end{equation}
\end{theorem}
Equation \eqref{eq:limit_lipschitz} underlines the dependence of the sum of the norm of the gradients on the variance of the gradients. The better the gradients are estimated, the closer one gets to the optimum where the gradient vanishes. As the dependence on the sample size becomes $\oo\left(N^{-1}\right)$ for a RQMC sequence instead of $1/N$ for a MC sequence, the gradient is more precisely estimated for $N$ large enough. We now study the impact of a reduced variance when applying the stochastic gradient descent with fixed stepsize to strongly convex functions. 

\begin{theorem} \label{theorem:strongly_convex_functions}
Let $F$ be a strongly convex function, e.g. there exists a constant $c>0$ s.t. $\forall \lambdavec, \overline{\lambdavec}$ $ \F(\overline{\lambdavec})  \geq \F(\lambdavec) + \nabla \F(\lambdavec)^T (\lambdavec -  \overline{\lambdavec}) + \frac{1}{2} c \norm{ \lambdavec - \overline{\lambdavec} }$, let $U_N = \{ \uvec_1, \cdots, \uvec_N \}$ be a RQMC sequence and let $ \forall \lambdavec$ $G: \uvec \rightarrow \nabla \F_{\Gamma(\uvec)}(\lambdavec)$ satisfy the conditions of Theorem \ref{theorem:owen}. Let $\alpha < \frac{1}{2c}$. Then the expected optimality gap satisfies 
\begin{eqnarray*}
\EE[\F_N(\lambdavec_{t+1}) - \F(\lambdavec^\star)] \leq  \left[ \left( \frac{\alpha^2 L}{2} - \alpha \right) 2c +1 \right ]\\ \times \EE[\F_N(\lambdavec_{t})  - \F(\lambdavec^\star)] \\ + \frac{1}{2} L \alpha^2 \left[ M_V r(N) \right]
\end{eqnarray*}
Consequently, 
\begin{equation} \label{eq:limit_strongly_convex}
\limT \EE[\F_N(\lambdavec_{T}) - \F(\lambdavec^\star)] \leq \frac{\alpha L }{4c - \alpha L c} \left[ M_V r(N) \right].
\end{equation}
\end{theorem}
The previous result has the following interpretation. The expected optimality gap between the last iteration $\lambdavec_T$ and the true minimizer $\lambdavec^\star$ is upper bounded by the magnitude of the variance. The more this variance gets reduced, the closer we get to the true point $\lambdavec^\star$. In this sense using an estimator with reduced variance is beneficial for the optimization routine. 

\subsection{Adaptive step size algorithms}
QMC applied to adam \cite{kingma2014adam}. Can upper bound of regret be improved? No results on accelerated convergence yet. Other approaches: linear convergence can be obtained if the mini batch sample size grows with each iteration for decreasing step size schedules, see \cite{bottou2016optimization}. For MC samples the mini batch sample size has to increase geometrically as $ N_t =  N \epsilon^t$ and $\epsilon > 1$. For (R)QMC this could be reduced to $  N_t \approx N \epsilon^{t/2}$. However, this is prohibitive in real applications. In practice when using (R)QMC instead of MC we observe improved convergence for adagrad and adam. 

\subsection{Stochastic gradient descent and mini batch sampling}
In the previous analysis we have assumed that the entire randomness in the gradient estimator comes from the sampling from the variational distribution. In practice additional randomness is introduced via mini batch sampling. This leads to a dominating term of order $N^{-1/2}$. The part of the variance related to the variational family is still reduced and thus the variance of the gradient estimator as a whole. 

==> preamble.tex <==
% FONTS
\usepackage[T1]{fontenc}

% Replace default Latin Modern typewriter with its proportional counterpart
% http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
\renewcommand*\ttdefault{lmvtt}

%%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

\usepackage{tgtermes}
\usepackage{amsmath}
%\usepackage[subscriptcorrection,
%            amssymbols,
%            mtpbb,
%            mtpcal,
%            nofontinfo  % suppresses all warnings
%           ]{mtpro2}
\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
\usepackage[scaled=0.92]{PTSans}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{framed}
\usepackage{nicefrac}

% EDITING
% line numbering in left margin
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}
% ragged paragraphs in right margin
\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}
% paragraph helper
\DeclareRobustCommand{\PP}{\textcolor{Plum}{\P}~}
\DeclareRobustCommand{\pp}{\textcolor{Plum}{\P}~}
\DeclareRobustCommand{\parhead}[1]{\vspace{0.05in} \textbf{#1} }

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
%\usepackage[format=hang]{subcaption}
\usepackage{subfig}

% TABLES
\usepackage{booktabs}
\usepackage{tabu}

% BIBLIOGRAPHY
\usepackage{natbib}

% ALGORITHMS
%\usepackage[algoruled]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=Violet}
\hypersetup{linkcolor=black}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}

% ACRONYMS
\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}
\crefname{appendix}{supplement}{}
% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\usepackage{listings}
\lstdefinestyle{alp_style}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=alp_style}

==> qmc_writeup.tex <==
\section{QMC Write up, previous comments flo}
\commentf{copy the stuff from here step by step to the methods section}

\subsection{Non-Conjugate VI, structure Flo}

\begin{itemize}
    \item Introduce problem variational inference + gradient estimator
    \item two popular methods: score function estimator (REINFORCE) and reparemeterization gradient
    \item both consist of approximating expectations w.r.t. to the variational distribution
    \item Quasi Monte Carlo methods deal with this setting of approximating an integral w.r.t. to a base measure (the variational distribution) and exhibit a faster convergence compared to standard Monte Carlo sampling
    \item using QMC for estimating the gradient leads  to lower variance estimators than the usual standard random sampling (MC) based methods (see theory section)
\end{itemize}


\subsection{QMCVI}

\commenta{check which parts still to use}
Using Monte Carlo samples \commentf{explain what MC samples mean. samples from an arbitrary correct sampler?} the estimators \eqref{eq:grad_estimators} are unbiased and converge to their expectations at a rate of $N^{-1/2}$. 
The obtained ELBO and gradient estimators can be used for stochastic optimization in order to find the maximum of the ELBO.
However, if the gradients exhibit high variance the gradient ascent might converge slowly. Schemes for reducing the gradient variance are for example Rao-Blackwellization, control variates or importance sampling. In this work we advocate the idea of using quasi Monte Carlo samples  for the generation of either $\varepsilon$ or $z$ that yield gradients with lower variance and hence improves the optimization routine. 
\begin{itemize}
    \item Emphasize that QMC is more like a meta technique for variance reduction and many other variance reduction methods as Rao-Blackwellization or importance sampling can be combined with it.
    \item (But for control variates it's not directly possible.)
\end{itemize}

Use RQMC in practice due to the unbiasedness property



\begin{itemize}
    \item Briefly explain the idea of QMC and low discrepancy sequences and give main efficiency results
    \item RQMC leads to unbiased gradient estimator and has lower variance than the standard MC approach
    \item insert order variance reduction (rate of error) here (which is opposed to $\mathcal{O}(N^{-\frac{1}{2}}$ using MC)
    \item in the theory section we show that using qmc in the setting of stochastic optimization leads to faster convergence rates
    \item we show it in the simplified case of sgd with constant learning rate but we observe empirically that qmc in combination with minibatch sampling and adaptive learning rate schemes also can speed up the algorithm
\end{itemize}

\paragraph{Generating Quasi Monte Carlo Samples}
\commentf{Could also be renamed in "Implementation Details" or "Algorithm".}
\begin{itemize}
    \item Which construction scheme do we use? \commenta{Construction based on inverse cumulative distribution function in 1 dimension, applied component wise, inverse cdf has to be sufficiently regular}
    \commentf{I actually meant generating the QMC sequence. Is it just a text file you with precomputed numbers?}
    \item what is the computational overhead? \commenta{Overhead in terms of the evaluation of the inverse cdf, depends on how the random variables are generated in detail}
     \item Practical considerations: For which distributions can we use QMC?
    \item explain for which models QMC can be used and emphasize that in combination with the score function estimator it's more general than reparemetrization
    \item It is straightforward to extend existing code by changing the random number generation process. \commenta{But we have to be careful: no direct application to MCMC based sampling}
\end{itemize}

\begin{itemize}
    \item we study the use of RQMC for stochastic optimization in general
    \item summarize main results
    \item Theorem 1 + 2: SGD with fixed step size
    \item comment on adaptive learning rate schemes and mini batch sampling (beyond the scope of our paper)
\end{itemize}

